On Hamiltonian Berge cycles in $3$-uniform hypergraphs

Given a set $R$, a hypergraph is $R$-uniform if the size of every hyperedge belongs to $R$. A hypergraph $\mathcal{H}$ is called \textit{covering} if every vertex pair is contained in some hyperedge in $\mathcal{H}$. In this note, we show that every covering $[3]$-uniform hypergraph on $n\geq 6$ vertices contains a Berge cycle $C_s$ for any $3\leq s\leq n$. As an application, we determine the maximum Lagrangian of $k$-uniform Berge-$C_{t}$-free hypergraphs and Berge-$P_{t}$-free hypergraphs.

==> revision.tex <==


Referee #2 (Remarks to the Author): 

S 


- Page 2, Line 1: In the definition of l-cycle in k-graphs, is a k-graph formed of two edges which share two vertices a 1-cycle with two edges? This is considered as a 1-cycle according to some authors, but this is not captured by your definition (which insists that the intersection of two consecutive edges should be exactly 1). Something similar can happen for l-cycles whenever 2l \leq k. 

- Page 2, Line 6: \delta as notation for the minimum degree in graphs has not been defined. 

- Page 2, Line 9: "In the setting of a hypergraph" -> "In the setting of hypergraphs,". 

- Page 2, Line 10: "every $k$-graph on $n$ vertices" should be "every $k$-graph $\mathcal{H}$ on $n$ vertices", since you use $\mathcal{H}$ to refer to the $k$-graph afterwards. 

- Page 2, Line 25: I don't understand the sentence beginning with "For Berge hypergraphs...". You haven't introduced what a "Berge hypergraph" is. I have not checked the paper that you cite, but if the result is simple to describe or if it is possible to describe the result in terms of the function \hat{h}_s(k, n) that you introduce later, I would do so. 

- Page 2, Line 27: Since every tight cycle also yields a Berge cycle on the same sequence of vertices, it would be useful to mention that the bounds on h^{k-1}_s(k,n) give bounds for \hat{h}_{s}(k, n). 

- Page 2, Line 30: Coulson and Perarnau ("A Rainbow Dirac's theorem", arxiv preprint, 2018) determine (in their Corollary 1.5) sufficient and sharp conditions about the existence of Berge cycles in k-graphs given lower bounds on $\delta_1(H)$, thus solving the problem of determining $\hat{h}_{1}(k, n)$. 

- Page 2, Theorem 1: The sentence after "In other words" is not precise, since the previous statement is for [k]-graphs and $\hat{h}_{s}(k, n) \ge 1$ is a statement only about k-graphs. Thus the statement about $\hat{h}_{s}(k, n)$ is implied by the previous statement, it is not the same statement with different words. 

- Page 2, Theorem 1: Note that if $s \ge 2$, then $\delta_s(H) > 0$ implies that $\delta_2(H) > 0$. Thus your result also implies that $s \ge 2$, $\hat{h}_{s}(k, n) <= 1$. Since the $s = 1$ case follows from the work of Coulson and Perarnau, you could mention that your result also determines (for large $n$) all of the degree thresholds for the existence of Hamiltonian Berge cycles, not just the 2-one. 

- Page 3, Line 1: The definition of trace makes perfect sense for all hypergraphs (not just $[k]$-graphs). Indeed is the case of general hypergraphs the one considered in some of the references you provide (dealing with the Vapnik-Chernovenkis-Perles-Sauer-Shelah lemma). It is then a (simple) observation that the trace of a $[k]$-graph is also a $[k]$-graph. The statement in Proposition 1 is also true for general hypergraphs. 

- Page 3, Line 3: "Trace of hypergraph is" should be "Traces of hypergraphs are". 

- Page 3, Proposition 1: "can be lifted" is not precise. I would state that there exists a Berge cycle or path in H for exactly the same sequence of vertices (and thus of the same length). 

- Page 3, Line 12: "using simply probabilistic" -> "using simple probabilistic". 

- Page 3, Proposition 2: "a Berge copy of G" is undefined. If this definition captures also the notion of Berge cycles and paths, then perhaps it would be useful to introduce this notion first, and then mention that Berge cycles and paths are "Berge copies" of the graph paths and cycles. 

- Page 3, Theorem 2: The proof of Theorem 2 is missing. I see how it can be deduced from Theorem 1 and Propositions 1-2, but it would be better to spell it out. 

- Page 3, Corollary 1: I think this is a Corollary of Theorem 1 instead, not of Theorem 2. 

- Page 3, after Corollary 1: It is strange to state the full content of Theorems 3 and 4 before the actual statement. I would say something along the lines "we can give more precise results whenever $k = 3$ or similar. 

- Page 3, Line 24: The bound on the number of edges of covering Berge-Hamiltonian 3-graphs is not true. For instance, the complete 3-graphs on 4, 5 or 6 vertices are covering and contain tight (hence, Berge) Hamilton cycles (hence, also Hamilton Berge paths). I see that you need at least n edges to have a Hamilton Berge cycle, and the fraction (n choose 2)/(3 choose 2) is a lower bound for the number of edges of a covering 3-graph on n vertices, but this bound is not necessarily attained, and it is _not_ an upper bound in general. Thus the small cases need to be revised. 

- Page 3, Line 24: I would also move the verification that the lower bounds in n in Theorems 3, 4 are best possible after the statements. 

- Page 3, Line 31: I would add more context to the conjectures. Are the conjectures tight (in n) for all k? Can you construct a particular example that you think is extremal, for each one of them? (that is, for Conjecture 2, a [k]-graph on k(k-1) vertices without a Hamilton Berge cycle). I have not thought about this in detail, but as a suggestion I would look at finite projective planes: those are minimally covering hypergraphs, they have the same number of vertices as edges, and the number of vertices is roughly the square of the size of the edges. Perhaps those hypergraphs, or alterations of them, give good examples. 

- Page 4, Line 1: In this page you repeat (at least three times) that you are going to apply the previous theorems to problems on Lagrangians. The first of these appears in Line 1, the second in Line 15, and then in Line 27 (just before Theorem 5). I would leave just one of them. 

- Page 4, Line 9: About the Lagrangian: as you notice, you might as well define the Lagrangian as the supremum only taken over non-negative vectors (and indeed is done like this in some sources), which might be clearer. Also perhaps it is useful to note that the "maximum" in the definition makes sense, since the optimization is taken over a compact set and the polynomials are continuous. 

- Page 4, Line 14: the phrase "useful in the Turán theory" sounds strange. 

- Page 4, Line 18: Typesetting: I would define a "math operator" for the extremal number, so "ex" does not appear italicised in math mode when you talk about Turán-type results. 

- Page 4, Line 18: "Berge-G-free hypergraph" is undefined (also what it means to have a "Berge" copy of some graph G). 

- Page 4, Line 32: Before presenting the Corollary, to aid the reader it would be helpful to indicate whether it follows immediately from Theorem 5 (so it does not deserve a detailed proof) or that the proof of the Corollary is detailed somewhere else. 

- Page 5, Line 16: "which defines the $o$, $O$ notation" is imprecise and unclear. Also it is used inconsistenly during the remainder of the section, since sometimes you use it to refer to asymptotics using large $n$ and sometimes it is used to refer to large $m$. 

- Page 5, Line 19: It would be helpful to show (or at least mention) that S^{(r)} corresponds exactly to the expectation of (X choose r). This is used afterwards and it would help to motivate the definitions. 

- Page 5, Theorem 6: The statement is very unclear. First: the inequalities in the math display in Line 22 hold for each n? 

- Page 5, Theorem 6: Second, since all of the variables depend on a hidden parameter n, in particular E[X] is a function on n. In Line 25, it is mentioned that S^{(r)} "converges" to some function of E[X]. I assume that this convergence happens when n goes to infinity. But what it worries me the most is that S^{(r)} is a function of n which converges, not to a fixed number, but to a sequence (since a priori E[X] varies with n). The notation of the "arrow" to indicate convergence in this case is non-standard and I think this would definitely need more clarification. As an observation, if E[X] should happen to converge (when n goes to infinity) to a constant, then the whole lemma would be only an easy consequence of the usual Brun's Sieve, as in your reference [2] (and it would not require to re-do the proof). 

- Page 6, Line 3: "Similar approach" -> "A similar approach". 

- Page 6, Line 3: Similarly as Theorem 6, it is not clear what the convergence means. 

- Page 6, Line 6: "e^{-x} is uniformly convergent" does not really make sense, since being "uniformly convergent" is a property of a sequence of functions, not of a single function. Alternatively you could say that e^{-x} is a real analytic function, so its Taylor series converges pointwise to e^{-x}, and thus uniformly over a compact. 

- Page 6, Line 12: It is not clear why the inequality in display (with S^{(r)} and E[X]^r/r!) holds since the "convergence" between them is not clear. 

- Page 6, Lines 20-23: The repetition could be avoided, you already introduced this setup before Theorem 6. 

- Page 7, Line 1: In the setup you have introduced, it is not necessary that m = m(n) is an increasing function of n. Thus the phrase "for each fixed integer r and sufficiently large m there exists c1, c2..." is not clear. The constants c1(r), c2(r) exist only when m is large? The inequalities hold only for large values of m? Similarly, in (5) and the following line you talk about o(1) or o(m^r) terms for "large values of m". This is unclear since the asymptotic notation, according to your setup, is taken with respect to n, not m. 

- Page 7, Lines 14-15: Going from the line with the sum of tuples of Type I and Type II to the next one, I think that you get an inequality instead of an equality (since you are using the upper bound of (4)). 

- Page 7, Lines 19-20: I am confused about the last two lines of the display, I think you are using (4) again but in that case it should also be an inequality. Further clarification for this part would be nice. 

- Page 8, Line 1: Similarly with the first equality of the page, I am confused as to why this is equality and not an inequality. 

- Page 8, Lines 3-4: More explanation is needed here as well. I am specially concerned about the sum over the tuples of Type I. That sum is not necessarily bounded in n or m, and it is multiplied by an o(1) (which is not clear if it is with respect to n or m), and it is deduced that the whole term is o(1). 

- Page 8, Line 7: "Let G be an arbitrary fixed graph" is redundant, since that appears in the statement of Proposition 2 already. But you do need to define what k is, since that does not appear in the statement of Proposition 2. 

- Page 8, Lines 10-11: "Since H is edge-minimal and covering, it follows that..." this is used multiple times during the paper, it might be worth to state this as a separate lemma or proposition (and give a proof). 

- Page 8, Line 4: I do not see how to get to the upper bound on Pr(B_i) given in the display. I can get a weaker upper bound which is still enough for the proof, but I would write more steps for that particular calculation. 

- Page 8, Line 17: It is not correct to say that a term "is o(1) when n is sufficiently large", since "being o(1)" is a property of a sequence of numbers (i.e. that it converges to 0), not of a particular value of n or large values of n. Also in this case it is enough to argue that for n sufficiently large the terms are less than 1. 

- Page 8, Line 19: "for every edge e \in E(G), there exists an hyperedge h(e) \in H such that e \subseteq h(e)" is strange, since e are edges of G which in principle are not a subgraph in the same vertices as H. I assume you are talking about copies. 

- Page 8, Line 19: As a small simplification for the proof, you might argue that it is enough to look for Berge copies of K_s, and use the property to find a "Berge copy" of K_s in the selected vertices. 

- Page 8, Lemma 1: "With probability at least e^{-k^4}" does not really make sense here, since the statement is deterministic. 

- Page 8, Lines 27-29: Maybe the construction can be more easily stated in terms of colourings: every pair uv of H is (greedily) assigned with a colour e_i such that uv \in e_i. 

- Page 9, Line 4: "uniformly randomly" -> "uniformly at random". 

- Page 9, Line 6: The description of the event B_i is unclear. Initially I thought that you required that the two vertex pairs e_1, e_2 needed to appear consecutively next each other, but it seems that you only want to capture the event that both pairs are represented in the cycle. I would change the presentation in this part. Since your objective is to build the Berge cycle by using precisely the order given by the (random) cyclic permutation that you choose, and the edge you have assigned for each pair, I would explicitly say so in this part. It might be helpful to notice that there are some authors that define "weak Hamilton cycles" which is like a Berge cycle but it might reuse edges of the hypergraph (see, e.g. Clemens, Ehrenmüller, Person, "A Dirac-type theorem for Hamilton Berge cycles in random hypergraphs", 2016). Thus, by the covering property, every permutation gives a "weak Hamilton cycle", and the objective is to show that with non-zero probability the cycle is actually Berge. And then B_i is the event that the "edge i" (or colour i, if you use colourings) is used at least twice in the cycle. 

- Page 9, Line 12, first display: I get why an upper bound holds for this, but the equality might require more explanation. 

- Page 9, Line 21, fifth display: I think more explanation would be needed for this. 

- Page 9, Line 21, sixth display: You seem to be using that m ~ n^2, I would explicitly mention or recall this. 

- Page 10, Line 4: the bound "m \leq (n choose 2)" uses that H is minimally covering (which is not being assumed at the moment). 

- Page 10, Line 9, fourth display: I would mention briefly what the notation \overline{S} means, since I think it has not been defined before. 

- Page 10, Line 14, fifth display: you are using edge-minimality of H again. Even if you were using it, the inequality is not immediate, since you are applying it to the subgraph induced on S \cup T_v, which might not even be covering (let alone minimally covering). 

- Page 10, Line 15, fifth display: perhaps using |S| \leq k n^{0.1} here would be useful. 

- Page 10, Line 18: the hypergraph you define corresponds precisely to the trace of H in \overline{S}, I would mention it. Then it would follow immediately that it is covering and that it is a [k]-graph from Proposition 1. 

- Page 10, Lines 19-24: it might be clearer to derive a direct upper bound for the set of (i,j) instead of proceeding by contradiction using the asymptotic notation. 

- Page 10, Line 21: Actually $|E(H_{\overline{S}}| \leq |E(H)| \leq \binom{n}{2}$, which is clearer. 

- Page 10, Line 26: the notation C = {u_1, ..., u_l} is not defined, and the notion of |C| when C is a Berge cycle is not defined either. It could also be helpful to say that C is a Berge cycle on |\overline{S}| vertices. 

- Page 10, Line 26: since you obtain the cycle in the "restricted" H_{\overline{S}}, you need "to lift" the cycle back to H (using Proposition 1) before proceeding with the following steps. 

- Page 10, Line 27: maybe the rest of the proof can be shortened somewhat. You could take a Berge cycle C' which covers all of \overline{S} and covers the maximal number of vertices of S as possible. By showing the existence of C, you have proved that the set of cycles with that property is non-empty, so this maximum is well-defined. If the optimal cycle C' covers all of S then you are done; otherwise you need to do the "increasing" step only once. 

- Page 11, Line 5, second display: I don't get why the first inequality is true. 

- Page 11, Line 8: This part is very confusing for me. The choice of u_p, u_q, u_{p+1}, u_{q+1} is crucial but it is not clear at all. WHERE are these vertices located, are they all in T'_{v_1}? Where do you use the property that |T| > n to find those vertices? It is also not clear to me why there exists an unused h such that ${u_{p+1}, u_{q+1}} \subseteq h$ (I see there exists at least one such edge just because H is covering, but I do not see why it is possible to choose an unused edge). 

- Page 11, Line 10: the choice of h_p, h_q must also be distinct from h. 


% - Page 11, Line 30: Given that a Berge path P uses t vertices, at most t-1 other vertices not in the path belong to "used" edges (since H is a [3]-graph). Thus, if t + (t-1) < n, we can extend the path by selecting one completely unused vertex and joining one of the end vertices with it (there exists an edge which contains them both, by the covering property). Thus if P is maximal, then t+(t-1) >= n must hold, i.e. t is at least the ceiling of (n+1)/2. This implies, in particular, that if n >= 6, a maximal Berge path has at least 4 vertices (instead of 3). 

% - Page 12, Line 11: actually the argument in the proof of Theorem 3 does not use any lower bound on the number of edges, only that the [3]-graph is covering. The argument works just as fine for n >= 4. Even more is true, for every covering [3]-graph on n >= 4 vertices, the number of edges is at least n-1. You have stated and used before that a covering [k]-graph has at least binom{n}{2} / \binom{k}{2} edges. For k = 3, and using that the number of edges is an integer, you get that in every [3]-graph on n vertices, the number of edges is at least the ceiling of binom{n}{2} / 3. For n >= 5 this easily implies the number of edges is at least n-1. For n = 4, suppose the number of edges in a covering [3]-graph is at most 2. No edge can have size at most 2, otherwise that leaves at least (4 choose 2) - 1 >= 5 pairs uncovered which is not possible to cover with a single edge. Thus all edges have size exactly 3. A given edge covers exactly three pairs and leaves exactly three pairs uncovered, but these uncovered pairs span 4 vertices, which is also not possible to cover with a single edge of size 3. Thus H has at least 3 = n-1 edges. 


- Page 15, Lines 22-24, first display: it would be helpful to indicate why the inequalities are true. I understand the first one would follow just by considering all of the possible k-sets, but we need that the xi are positive to have the inequality (which we are NOT assuming since the xi are just reals, but it should be assumed, or added to the definition of Lagrangian). For the second inequality you used that the maximum is attained when all of the xi are equal and positive, but an explanation is needed. 


- Page 15, Proofs: Perhaps the proof might be streamlined with an auxiliary lemma to say that (under the appropriate hypothesis) if H does not have a Berge cycle or path on t vertices then the size of the largest I such that H is covering satisfies |I| < t; and another that says that if the largest I such that H is covering satisfies |I| = t then the Lagrangian is at most lambda(K^k_{t-1}). This would yield the proof of all of the "lagrangian" results in a more unified way. 

- Page 16, Lines 3-14: These cases should be revised according to the previous comments on the validity of Theorem 3 and 4 for smaller values of n. 




